Learning Hierarchical Visual Representations in Deep Neural Networks Using Hierarchical Linguistic Labels

Modern convolutional neural networks (CNNs) are able to achieve human-level object classification accuracy on specific tasks, and currently outperform competing models in explaining complex human visual representations. However, the categorization problem is posed differently for these networks than for humans: the accuracy of these networks is evaluated by their ability to identify single labels assigned to each image. These labels often cut arbitrarily across natural psychological taxonomies (e.g., dogs are separated into breeds, but never jointly categorized as "dogs"), and bias the resulting representations. By contrast, it is common for children to hear both "dog" and "Dalmatian" to describe the same stimulus, helping to group perceptually disparate objects (e.g., breeds) into a common mental class. In this work, we train CNN classifiers with multiple labels for each image that correspond to different levels of abstraction, and use this framework to reproduce classic patterns that appear in human generalization behavior.

==> 08-discussion.tex <==
\section{Discussion}

\todo{{\bf NOTE -- I moved this from the intro. We can integrate some of it here and remove the rest.} -- Recent work in explainable AI has emphasized the importance of understanding the biases that the training data or a model's architecture can introduce \citep[\eg,][]{zhao2017men, ritter2017cognitive}. 
\an{This is in the background section now. Maybe mention here.}
\an{Add discussion about why basic=basic+sub}
%
Our analysis sheds light on another one of these important biases -- the basic-level bias -- that this image classification model captures. The model, even when trained on single labels, to some extent generalize a novel label to the basic-level category.
%
Finally, our results shows the importance of considering the right level of generalization and the choice of number of labels in image classification applications.}

Image classification models are often trained on images paired with single labels that correspond to the subordinate level of the hierarchical taxonomy. People, on the other hand, use multiple labels to refer to the same entity in the world (\eg, dog and Dalmatian). This explicit use of multiple labels makes the category learning problem easier as people can use the labels to identify similarities between the concepts (in addition to other features, such as perceptual cues, that signal similarity).
%
Moreover, the use multiple labels helps form hierarchical representations that capture different levels of abstraction. For example, two Dalmatians are more similar to each other than a Dalmatian to a poodle; dalmatians and poodles are still highly similar and should share more representations than a Dalmatian and a cow.
%
This hierarchical nature of the representation is in turn helpful in categorizing and labeling a new entity -- a problem that is often formulated as a few or one shot learning task in machine learning.
%
A child can use the similarity of an unobserved breed of dog (a Great Pyrenees) to previously-seen dogs to categorize and infer a label for it.

However, to our knowledge, none of the existing modern image classification models simultaneously train on multiple labels.
In this paper, we show that training on basic-level and sub-ordinate labels (or just basic-level labels) results in representations that better capture the hierarchical structure of taxonomy of real-world objects.
%
We also show that these representations result better match the basic-level bias observed in human generalization behavior.

Interestingly, we observe that a relatively big portion of ImageNet ($10\%$) are subordinate dog labels. Future work should look at other datasets with more interesting, less skewed basic label stratifications. Additionally, we only explore basic and subordinate levels in this work, which are both known to share many features in common with their members \cite{rosch.1978}, whereas high-level superordinate classes (e.g., furniture) often have members with few shared features. Including this type of pressure on the representation, and other arbitrary higher-level sets will make for interesting pressures on the representation space. 

Further, we only explore human-like generalization here, but it will be worth examining if representations that embody structured taxonomies can aid existing few-shot learning methods in machine learning, an approach that has been left generally unexplored despite being the focus on research with humans for a number of years.

%Future work needs to investigate whether these representations result in performance in 


%\an{We should compare this result with and with label. The importance of language in learning rep.}
